Optimal Trade Execution with Uncertain Volume Target

In the seminal paper on optimal execution of portfolio transactions, Almgren and Chriss (2001) define the optimal trading strategy to liquidate a fixed volume of a single security under price uncertainty. Yet there exist situations, such as in the power market, in which the volume to be traded can only be estimated and becomes more accurate when approaching a specified delivery time. During the course of execution, a trader should then constantly adapt their trading strategy to meet their fluctuating volume target. In this paper, we develop a model that accounts for volume uncertainty and we show that a risk-averse trader has benefit in delaying their trades. More precisely, we argue that the optimal strategy is a trade-off between early and late trades in order to balance risk associated with both price and volume. By incorporating a risk term related to the volume to trade, the static optimal strategies suggested by our model avoid the explosion in the algorithmic complexity usually associated with dynamic programming solutions, all the while yielding competitive performance.

==> images/tikz/analysis_demand_forecast_source_files/analysis_demand_forecast_im0.tex <==
\begin{tikzpicture}
  \begin{axis}[
    x dir=reverse,
    xmajorgrids,
    ymajorgrids,
    width=12cm,height=7cm,
    xmin=0,
    xmax=48.5,
    xtick={0,4,9,14,19,24,29,34,39,44,48},
    xticklabels={0 \\ $(T)$, 4 \\ ($\tau_{45}$), 9 \\ ($\tau_{40}$), 14 \\ ($\tau_{35}$), 19 \\ ($\tau_{30}$), 24 \\ ($\tau_{25}$), 29 \\ ($\tau_{20}$), 34 \\ ($\tau_{15}$), 39 \\ ($\tau_{10}$), 44 \\ ($\tau_{5}$), 48 \\ ($\tau_{1}$)},
    xticklabel style={align=center},
    % title = Mean Absolute Relative Forecast Error,
    title = Mean Relative Forecast Error,
    xlabel = Number of half-hours ahead of the settlement period,
    ylabel = Proportion of $\rtargetsum_{T}$ in \%,
    legend pos=south west,
    legend entries={
      Data points,
      Polynomial approximation,
    },
    legend cell align={left},
    every axis plot/.append style={ultra thick}
    ]
    \addplot[color=Paired-F,only marks,mark size=1.0pt] table [x expr=\thisrow{TimeHorizon},y expr=100*\thisrow{MeanAbsRelative}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/forecast_error/1825/NDF_forecast_error_ndaysdata_1825.txt};
    \addplot[color=Paired-D,mark=none,very thick] table [x expr=\thisrow{TimeHorizon},y expr=100*\thisrow{MeanAbsRelative}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/forecast_error/1825/NDF_polynomial_approximation_forecast_error_ndaysdata_1825.txt};
  \end{axis}
\end{tikzpicture}


==> images/tikz/analysis_demand_forecast_source_files/analysis_demand_forecast_im1.tex <==
\begin{tikzpicture}
  \begin{axis}[
    x dir=reverse,
    xmajorgrids,
    ymajorgrids,
    width=12cm,height=7cm,
    xmin=0,
    xmax=48.5,
    xtick={0, 4,9,14,19,24,29,34,39,44,48},
    xticklabels={0 \\ $(T)$, 4 \\ ($\tau_{45}$), 9 \\ ($\tau_{40}$), 14 \\ ($\tau_{35}$), 19 \\ ($\tau_{30}$), 24 \\ ($\tau_{25}$), 29 \\ ($\tau_{20}$), 34 \\ ($\tau_{15}$), 39 \\ ($\tau_{10}$), 44 \\ ($\tau_{5}$), 48 \\ ($\tau_{1}$)},
    xticklabel style={align=center},
    title = Standard Deviation of the Absolute Relative Forecast Error,
    xlabel = Number of half-hours ahead of the settlement period,
    ylabel = Proportion of $\rtargetsum_{T}$ in \%,
    legend pos=south west,
    legend entries={
      Data points,
      Polynomial approximation,
    },
    legend cell align={left},
    every axis plot/.append style={ultra thick}
    ]
    \addplot[color=Paired-F,only marks,mark size=1.0pt] table [x expr=\thisrow{TimeHorizon},y expr=100*\thisrow{StdAbsRelative}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/forecast_error/1825/NDF_forecast_error_ndaysdata_1825.txt};
    \addplot[color=Paired-D,mark=none,very thick] table [x expr=\thisrow{TimeHorizon},y expr=100*\thisrow{StdAbsRelative}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/forecast_error/1825/NDF_polynomial_approximation_forecast_error_ndaysdata_1825.txt};
  \end{axis}
\end{tikzpicture}


==> images/tikz/analysis_demand_forecast_source_files/analysis_demand_forecast_im2.tex <==
\begin{tikzpicture}
  \begin{axis}[
    x dir=reverse,
    xmajorgrids,
    ymajorgrids,
    width=12cm,height=7cm,
    xmin=0,
    xmax=48.5,
    xtick={0, 4,9,14,19,24,29,34,39,44,48},
    xticklabels={0 \\ $(T)$, 4 \\ ($\tau_{45}$), 9 \\ ($\tau_{40}$), 14 \\ ($\tau_{35}$), 19 \\ ($\tau_{30}$), 24 \\ ($\tau_{25}$), 29 \\ ($\tau_{20}$), 34 \\ ($\tau_{15}$), 39 \\ ($\tau_{10}$), 44 \\ ($\tau_{5}$), 48 \\ ($\tau_{1}$)},
    xticklabel style={align=center},
    title = Mean of the Relative Forecast Update,
    xlabel = Number of half-hours ahead of the settlement period,
    ylabel = Proportion of $\rtargetsum_{T}$ in \%,
    legend pos=south west,
    legend entries={
      Data points,
      Polynomial approximation,
    },
    legend cell align={left},
    every axis plot/.append style={ultra thick},
    scaled ticks=false,
    tick label style={/pgf/number format/fixed} 
    ]
    \addplot[color=Paired-F,only marks,mark size=1.0pt] table [x expr=\thisrow{TimeHorizon},y expr=100*\thisrow{MeanRelative}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/forecast_update/1825/NDF_forecast_update_ndaysdata_1825.txt};
    \addplot[color=Paired-D,mark=none,very thick] table [x expr=\thisrow{TimeHorizon},y expr=100*\thisrow{MeanRelative}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/forecast_update/1825/NDF_polynomial_approximation_forecast_update_ndaysdata_1825.txt};
  \end{axis}
\end{tikzpicture}


==> images/tikz/analysis_demand_forecast_source_files/analysis_demand_forecast_im3.tex <==
\begin{tikzpicture}
  \begin{axis}[
    x dir=reverse,
    xmajorgrids,
    ymajorgrids,
    width=12cm,height=7cm,
    xmin=0,
    xmax=48.5,
    xtick={0, 4,9,14,19,24,29,34,39,44,48},
    xticklabels={0 \\ $(T)$, 4 \\ ($\tau_{45}$), 9 \\ ($\tau_{40}$), 14 \\ ($\tau_{35}$), 19 \\ ($\tau_{30}$), 24 \\ ($\tau_{25}$), 29 \\ ($\tau_{20}$), 34 \\ ($\tau_{15}$), 39 \\ ($\tau_{10}$), 44 \\ ($\tau_{5}$), 48 \\ ($\tau_{1}$)},
    xticklabel style={align=center},
    title = Standard Deviation of the Relative Forecast Update,
    xlabel = Number of half-hours ahead of the settlement period,
    ylabel = Proportion of $\rtargetsum_{T}$ in \%,
    legend pos=north west,
    legend entries={
      Data points,
      Polynomial approximation,
    },
    legend cell align={left},
    every axis plot/.append style={ultra thick}
    ]
    \addplot[color=Paired-F,only marks,mark size=1.0pt] table [x expr=\thisrow{TimeHorizon},y expr=100*\thisrow{StdRelative}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/forecast_update/1825/NDF_forecast_update_ndaysdata_1825.txt};
    \addplot[color=Paired-D,mark=none,very thick] table [x expr=\thisrow{TimeHorizon},y expr=100*\thisrow{StdRelative}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/forecast_update/1825/NDF_polynomial_approximation_forecast_update_ndaysdata_1825.txt};
  \end{axis}
\end{tikzpicture}


==> images/tikz/analysis_demand_forecast_source_files/analysis_demand_forecast_im4.tex <==
\begin{tikzpicture}
  \begin{axis}[
    x dir=reverse,
    xmajorgrids,
    ymajorgrids,
    width=12cm,height=7cm,
    xmin=0,
    xmax=48.5,
    xtick={0, 4,9,14,19,24,29,34,39,44,48},
    xticklabels={0 \\ $(T)$, 4 \\ ($\tau_{45}$), 9 \\ ($\tau_{40}$), 14 \\ ($\tau_{35}$), 19 \\ ($\tau_{30}$), 24 \\ ($\tau_{25}$), 29 \\ ($\tau_{20}$), 34 \\ ($\tau_{15}$), 39 \\ ($\tau_{10}$), 44 \\ ($\tau_{5}$), 48 \\ ($\tau_{1}$)},
    xticklabel style={align=center},
    title = Probability Forecast Update,
    xlabel = Number of half-hours ahead of the settlement period,
    ylabel = Probability,
    legend pos=north east,
    legend entries={
      Data points,
      Polynomial approximation,
    },
    legend cell align={left},
    every axis plot/.append style={ultra thick},
    scaled ticks=false,
    tick label style={/pgf/number format/fixed} 
    ]
    \addplot[color=Paired-F,only marks,mark size=1.0pt] table [x expr=\thisrow{TimeHorizon},y expr=\thisrow{ProbUpdate}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/forecast_update/1825/NDF_forecast_update_ndaysdata_1825.txt};
    \addplot[color=Paired-D,mark=none,very thick] table [x expr=\thisrow{TimeHorizon},y expr=\thisrow{ProbUpdate}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/forecast_update/1825/NDF_polynomial_approximation_forecast_update_ndaysdata_1825.txt};
  \end{axis}
\end{tikzpicture}


==> images/tikz/distribution_power_update_source_files/distribution_power_update_im0.tex <==
% --------------------------
% - Risk-aversion λ = 0.25 -
% --------------------------
% Mean CVaR (PU): 
% 	pdf_13918139747969224024.txt
% 	cdf_13918139747969224024.txt
% Mean CVaR (PVU): 
% 	pdf_10153472541130893391.txt
% 	cdf_10153472541130893391.txt

\begin{tikzpicture}
  \begin{axis}[
    xmajorgrids,width=12cm,height=7cm,
    ymajorgrids,
    xmin = -1 * 10.0^6,
    xmax = 5*10^6,
    ymin = 0.0*10^-6,
    % ymax = 0.08,
    y tick label style={
      /pgf/number format/.cd,
      fixed,
      fixed zerofill,
      precision=1,
      /tikz/.cd
    },
    xlabel = Trading cost,
    % ylabel = Proportion to trade,
    legend pos=north east,
    legend entries={
      Mean-$\CVaR_{0.1}$ (PU),
      Mean-$\CVaR_{0.1}$ (PVU),
    },
    legend cell align={left},
    every axis plot/.append style={ultra thick}
    ]
    \pgfplotsset{cycle list set=2}
    \addplot table [x=x,y=y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/pdf_13918139747969224024.txt};
    \addplot table [x=x,y=y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/pdf_10153472541130893391.txt};
  \end{axis}
  % \node[above,font=\large\bfseries] at (current bounding box.north) {$\lambda_{\CVaR} = 0.25$};
\end{tikzpicture}


==> images/tikz/distribution_power_update_source_files/distribution_power_update_im1.tex <==
% --------------------------
% - Risk-aversion λ = 0.5 -
% --------------------------
% Mean CVaR (PU): 
% 	pdf_12075258543483517010.txt
% 	cdf_12075258543483517010.txt
% Mean CVaR (PVU): 
% 	pdf_17233269158857089779.txt
% 	cdf_17233269158857089779.txt

\begin{tikzpicture}
  \begin{axis}[
    xmajorgrids,width=12cm,height=7cm,
    ymajorgrids,
    xmin = -1 * 10.0^6,
    xmax = 5*10^6,
    ymin = 0.0*10^-6,
    % ymax = 0.08,
    y tick label style={
      /pgf/number format/.cd,
      fixed,
      fixed zerofill,
      precision=1,
      /tikz/.cd
    },
    xlabel = Trading cost,
    % ylabel = Proportion to trade,
    legend pos=north east,
    legend entries={
      Mean-$\CVaR_{0.1}$ (PU),
      Mean-$\CVaR_{0.1}$ (PVU),
    },
    legend cell align={left},
    every axis plot/.append style={ultra thick}
    ]
    \pgfplotsset{cycle list set=2}
    \addplot table [x=x,y=y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/pdf_12075258543483517010.txt};
    \addplot table [x=x,y=y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/pdf_17233269158857089779.txt};
  \end{axis}
  % \node[above,font=\large\bfseries] at (current bounding box.north) {$\lambda_{\CVaR} = 0.25$};
\end{tikzpicture}


==> images/tikz/distribution_power_update_source_files/distribution_power_update_im2.tex <==
% --------------------------
% - Risk-aversion λ = 0.75 -
% --------------------------
% Mean CVaR (PU): 
% 	pdf_2695718419451503433.txt
% 	cdf_2695718419451503433.txt
% Mean CVaR (PVU): 
% 	pdf_1747615791120220393.txt
% 	cdf_1747615791120220393.txt

\begin{tikzpicture}
  \begin{axis}[
    xmajorgrids,width=12cm,height=7cm,
    ymajorgrids,
    xmin = -1 * 10.0^6,
    xmax = 5*10^6,
    ymin = 0.0*10^-6,
    % ymax = 0.08,
    y tick label style={
      /pgf/number format/.cd,
      fixed,
      fixed zerofill,
      precision=1,
      /tikz/.cd
    },
    xlabel = Trading cost,
    % ylabel = Proportion to trade,
    legend pos=north east,
    legend entries={
      Mean-$\CVaR_{0.1}$ (PU),
      Mean-$\CVaR_{0.1}$ (PVU),
    },
    legend cell align={left},
    every axis plot/.append style={ultra thick}
    ]
    \pgfplotsset{cycle list set=2}
    \addplot table [x=x,y=y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/pdf_2695718419451503433.txt};
    \addplot table [x=x,y=y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/pdf_1747615791120220393.txt};
  \end{axis}
  % \node[above,font=\large\bfseries] at (current bounding box.north) {$\lambda_{\CVaR} = 0.25$};
\end{tikzpicture}


==> images/tikz/distribution_power_update_source_files/distribution_power_update_im3.tex <==
% --------------------------
% - Risk-aversion λ = 1.0 -
% --------------------------
% Mean CVaR (PU): 
% 	pdf_18202928793810891683.txt
% 	cdf_18202928793810891683.txt
% Mean CVaR (PVU): 
% 	pdf_16915398136104719935.txt
% 	cdf_16915398136104719935.txt

\begin{tikzpicture}
  \begin{axis}[
    xmajorgrids,width=12cm,height=7cm,
    ymajorgrids,
    xmin = -1 * 10.0^6,
    xmax = 5*10^6,
    ymin = 0.0*10^-6,
    % ymax = 0.08,
    y tick label style={
      /pgf/number format/.cd,
      fixed,
      fixed zerofill,
      precision=1,
      /tikz/.cd
    },
    xlabel = Trading cost,
    % ylabel = Proportion to trade,
    legend pos=north east,
    legend entries={
      Mean-$\CVaR_{0.1}$ (PU),
      Mean-$\CVaR_{0.1}$ (PVU),
    },
    legend cell align={left},
    every axis plot/.append style={ultra thick}
    ]
    \pgfplotsset{cycle list set=2}
    \addplot table [x=x,y=y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/pdf_18202928793810891683.txt};
    \addplot table [x=x,y=y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/pdf_16915398136104719935.txt};
  \end{axis}
  % \node[above,font=\large\bfseries] at (current bounding box.north) {$\lambda_{\CVaR} = 0.25$};
\end{tikzpicture}


==> images/tikz/mean_cvar_strat_diff_liquidity_source_files/mean_cvar_strat_diff_liquidity_im0.tex <==
%%%%%%%%%%%%%%%%%%
% Mean-CVaR (PU) %
%%%%%%%%%%%%%%%%%%

% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_1752420666672134910.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_5450853095578913331.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_15064030181349527357.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_11087128594625601859.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_17388827052995296055.jld2

\begin{tikzpicture}
  \begin{axis}[
    ymin = -0.1,
    ymax = 1.05,
    xtick={1,2,3,4,5},
    xticklabels={$\tau_{1}$,$\tau_{2}$,$\tau_{3}$,$\tau_{4}$,$\tau_{5}$},
    xmajorgrids,
    ymajorgrids,
    xlabel = Trading period,
    ylabel = Proportion to trade,
    legend pos=north east,
    legend entries={
      $\lambda_{\CVaR} = 0.00$,
      $\lambda_{\CVaR} = 0.25$,
      $\lambda_{\CVaR} = 0.50$,
      $\lambda_{\CVaR} = 0.75$,
      $\lambda_{\CVaR} = 1.00$,
    },
    legend style={nodes={scale=0.9, transform shape}}, 
    every axis plot/.append style={ultra thick},
    ]
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_1752420666672134910.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_5450853095578913331.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_15064030181349527357.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_11087128594625601859.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_17388827052995296055.txt};
  \end{axis}
\end{tikzpicture}


==> images/tikz/mean_cvar_strat_diff_liquidity_source_files/mean_cvar_strat_diff_liquidity_im1.tex <==
%%%%%%%%%%%%%%%%%%%
% Mean-CVaR (PVU) %
%%%%%%%%%%%%%%%%%%%

% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_4334348521088226683.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_5279361045231687549.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_4688433003597909411.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_1352773288804764848.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_1238960800518489720.jld2

\begin{tikzpicture}
  \begin{axis}[
    ymin = -0.1,
    ymax = 1.05,
    xtick={1,2,3,4,5},
    xticklabels={$\tau_{1}$,$\tau_{2}$,$\tau_{3}$,$\tau_{4}$,$\tau_{5}$},
    xmajorgrids,
    ymajorgrids,
    xlabel = Trading period,
    ylabel = Proportion to trade,
    legend pos=north east,
    legend entries={
      $\lambda_{\CVaR} = 0.00$,
      $\lambda_{\CVaR} = 0.25$,
      $\lambda_{\CVaR} = 0.50$,
      $\lambda_{\CVaR} = 0.75$,
      $\lambda_{\CVaR} = 1.00$,
    },
    legend style={nodes={scale=0.9, transform shape}}, 
    every axis plot/.append style={ultra thick},
    ]
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_4334348521088226683.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_5279361045231687549.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_4688433003597909411.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_1352773288804764848.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_1238960800518489720.txt};
  \end{axis}
\end{tikzpicture}



==> images/tikz/mean_cvar_strat_diff_liquidity_source_files/mean_cvar_strat_diff_liquidity_im2.tex <==
%%%%%%%%%%%%%%%%%%
% Mean-CVaR (PU) %
%%%%%%%%%%%%%%%%%%

% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_1752420666672134910.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_5450853095578913331.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_15064030181349527357.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_11087128594625601859.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_17388827052995296055.jld2

%%%%%%%%%%%%%%%%%%%
% Mean-CVaR (PVU) %
%%%%%%%%%%%%%%%%%%%

% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_4334348521088226683.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_5279361045231687549.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_4688433003597909411.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_1352773288804764848.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_1238960800518489720.jld2

%%%%%%%%%%%%%%%
%% Difference %
%%%%%%%%%%%%%%%

\begin{tikzpicture}
  \begin{axis}[
    ymin = -0.22,
    ymax = 0.22,
    ytick={-0.2,-0.15,-0.1,-0.05,0.0,0.05,0.1,0.15,0.2},
    yticklabels={-0.2,-0.15,-0.1,-0.05,0.0,0.05,0.1,0.15,0.2},
    xtick={1,2,3,4,5},
    xticklabels={$\tau_{1}$,$\tau_{2}$,$\tau_{3}$,$\tau_{4}$,$\tau_{5}$},
    xmajorgrids,
    ymajorgrids,
    xlabel = Trading period,
    ylabel = Proportion to trade,
    legend pos=north east,
    legend entries={
      $\lambda_{\CVaR} = 0.00$,
      $\lambda_{\CVaR} = 0.25$,
      $\lambda_{\CVaR} = 0.50$,
      $\lambda_{\CVaR} = 0.75$,
      $\lambda_{\CVaR} = 1.00$,
    },
    legend style={nodes={scale=0.9, transform shape}}, 
    every axis plot/.append style={ultra thick},
    ]
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_1752420666672134910_mean-cvar-optim_4334348521088226683.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_5450853095578913331_mean-cvar-optim_5279361045231687549.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_15064030181349527357_mean-cvar-optim_4688433003597909411.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_11087128594625601859_mean-cvar-optim_1352773288804764848.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_17388827052995296055_mean-cvar-optim_1238960800518489720.txt};
  \end{axis}
\end{tikzpicture}


==> images/tikz/mean_cvar_strat_uniform_liquidity_source_files/mean_cvar_strat_uniform_liquidity_im0.tex <==
%%%%%%%%%%%%%%%%%%
% Mean-CVaR (PU) %
%%%%%%%%%%%%%%%%%%

% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_793823805462494186.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_16314307504654312620.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_7504924619921099156.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_12709768837188935690.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_2275215992570049948.jld2

\begin{tikzpicture}
  \begin{axis}[
    ymin = -0.1,
    ymax = 1.05,
    xtick={1,2,3,4,5},
    xticklabels={$\tau_{1}$,$\tau_{2}$,$\tau_{3}$,$\tau_{4}$,$\tau_{5}$},
    xmajorgrids,
    ymajorgrids,
    xlabel = Trading period,
    ylabel = Proportion to trade,
    legend pos=north east,
    legend entries={
      $\lambda_{\CVaR} = 0.00$,
      $\lambda_{\CVaR} = 0.25$,
      $\lambda_{\CVaR} = 0.50$,
      $\lambda_{\CVaR} = 0.75$,
      $\lambda_{\CVaR} = 1.00$,
    },
    legend style={nodes={scale=0.9, transform shape}}, 
    every axis plot/.append style={ultra thick},
    ]
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_793823805462494186.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_16314307504654312620.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_7504924619921099156.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_12709768837188935690.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_2275215992570049948.txt};
  \end{axis}
\end{tikzpicture}


==> images/tikz/mean_cvar_strat_uniform_liquidity_source_files/mean_cvar_strat_uniform_liquidity_im1.tex <==
%%%%%%%%%%%%%%%%%%%
% Mean-CVaR (PVU) %
%%%%%%%%%%%%%%%%%%%

% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_17312322986288527794.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_17066045988445680639.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_17902867011452722062.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_15905289391306834247.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_12082414366513449257.jld2

\begin{tikzpicture}
  \begin{axis}[
    ymin = -0.1,
    ymax = 1.05,
    xtick={1,2,3,4,5},
    xticklabels={$\tau_{1}$,$\tau_{2}$,$\tau_{3}$,$\tau_{4}$,$\tau_{5}$},
    xmajorgrids,
    ymajorgrids,
    xlabel = Trading period,
    ylabel = Proportion to trade,
    legend pos=north east,
    legend entries={
      $\lambda_{\CVaR} = 0.00$,
      $\lambda_{\CVaR} = 0.25$,
      $\lambda_{\CVaR} = 0.50$,
      $\lambda_{\CVaR} = 0.75$,
      $\lambda_{\CVaR} = 1.00$,
    },
    legend style={nodes={scale=0.9, transform shape}}, 
    every axis plot/.append style={ultra thick},
    ]
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_17312322986288527794.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_17066045988445680639.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_17902867011452722062.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_15905289391306834247.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_12082414366513449257.txt};
  \end{axis}
\end{tikzpicture}


==> images/tikz/mean_cvar_strat_uniform_liquidity_source_files/mean_cvar_strat_uniform_liquidity_im2.tex <==
%%%%%%%%%%%%%%%%%%
% Mean-CVaR (PU) %
%%%%%%%%%%%%%%%%%%

% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_793823805462494186.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_16314307504654312620.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_7504924619921099156.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_12709768837188935690.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_2275215992570049948.jld2

%%%%%%%%%%%%%%%%%%%
% Mean-CVaR (PVU) %
%%%%%%%%%%%%%%%%%%%

% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_17312322986288527794.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_17066045988445680639.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_17902867011452722062.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_15905289391306834247.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_12082414366513449257.jld2

%%%%%%%%%%%%%%
% Difference %
%%%%%%%%%%%%%%

\begin{tikzpicture}
  \begin{axis}[
    ymin = -0.22,
    ymax = 0.22,
    ytick={-0.2,-0.15,-0.1,-0.05,0.0,0.05,0.1,0.15,0.2},
    yticklabels={-0.2,-0.15,-0.1,-0.05,0.0,0.05,0.1,0.15,0.2},
    xtick={1,2,3,4,5},
    xticklabels={$\tau_{1}$,$\tau_{2}$,$\tau_{3}$,$\tau_{4}$,$\tau_{5}$},
    xmajorgrids,
    ymajorgrids,
    xlabel = Trading period,
    ylabel = Proportion to trade,
    legend pos=north east,
    legend entries={
      $\lambda_{\CVaR} = 0.00$,
      $\lambda_{\CVaR} = 0.25$,
      $\lambda_{\CVaR} = 0.50$,
      $\lambda_{\CVaR} = 0.75$,
      $\lambda_{\CVaR} = 1.00$,
    },
    legend style={nodes={scale=0.9, transform shape}}, 
    every axis plot/.append style={ultra thick},
    ]
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_793823805462494186_mean-cvar-optim_17312322986288527794.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_16314307504654312620_mean-cvar-optim_17066045988445680639.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_7504924619921099156_mean-cvar-optim_17902867011452722062.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_12709768837188935690_mean-cvar-optim_15905289391306834247.txt};
    \addplot table [x=T,y=Y] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_2275215992570049948_mean-cvar-optim_12082414366513449257.txt};
  \end{axis}
\end{tikzpicture}


==> images/tikz/strategy_power_update_source_files/strategy_power_update_im0.tex <==
%%%%%%%%%%%%%%%%%%
% Mean-CVaR (PU) %
%%%%%%%%%%%%%%%%%%

% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_12345592210445333749.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_7754849124706072148.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_12944883113089842232.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_5114899910098603249.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_549416532610642337.jld2

\begin{tikzpicture}[]
  \begin{groupplot}[
    group style={
        group name=my fancy plots,
        group size=1 by 2,
        xticklabels at=edge bottom,
        vertical sep=0pt
    },
    xtick={1,5,10,15,20,25,30,35,40,47},
    xticklabels={$\tau_{1}$,$\tau_{5}$,$\tau_{10}$,$\tau_{15}$,$\tau_{20}$,$\tau_{25}$,$\tau_{30}$,$\tau_{35}$,$\tau_{40}$,$\tau_{47}$},
    ]

    \nextgroupplot[
    ymin = 0.018, ymax = 0.025,
    xmin = 0, xmax = 48,
    ytick={0.02,0.022,0.024},
    yticklabels={0.02,0.022,0.024},
    xmajorgrids, ymajorgrids,
    scaled ticks=false,
    yticklabel style={
      /pgf/number format/fixed,
      /pgf/number format/precision=5
    },
    y label style={at={(-0.12,0.4)}},
    axis x line=top, 
    axis y discontinuity=parallel,
    height=5.5cm,
    ylabel = Proportion to trade,
    xtick style={draw opacity=0},
    ] 

    \addplot table [x=T,y=Y,select coords between index={0}{45}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_12345592210445333749.txt};
    \addplot table [x=T,y=Y,select coords between index={0}{45}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_7754849124706072148.txt};
    \addplot table [x=T,y=Y,select coords between index={0}{45}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_12944883113089842232.txt};
    \addplot table [x=T,y=Y,select coords between index={0}{45}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_5114899910098603249.txt};
    \addplot table [x=T,y=Y,select coords between index={0}{45}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_549416532610642337.txt};

    \nextgroupplot[
    ymin = 0.0062, ymax = 0.0078,
    xmin = 0, xmax = 48,
    xmajorgrids, ymajorgrids,
    ytick={0.0065,0.007,0.0075},
    yticklabels={0.0065,0.007,0.0075},
    scaled ticks=false,
    yticklabel style={
      /pgf/number format/fixed,
      /pgf/number format/precision=5
    },
    legend pos=south west,
    legend entries={
      $\lambda_{\CVaR} = 0.00$,
      $\lambda_{\CVaR} = 0.25$,
      $\lambda_{\CVaR} = 0.50$,
      $\lambda_{\CVaR} = 0.75$,
      $\lambda_{\CVaR} = 1.00$,
    },
    legend style={at={(0.05,1.0)},anchor=west},
    axis x line=bottom,
    height=3.0cm,
    xlabel = Trading period,
    ]

    \addplot table [x=T,y=Y,select coords between index={46}{46}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_12345592210445333749.txt};
    \addplot table [x=T,y=Y,select coords between index={46}{46}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_7754849124706072148.txt};
    \addplot table [x=T,y=Y,select coords between index={46}{46}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_12944883113089842232.txt};
    \addplot table [x=T,y=Y,select coords between index={46}{46}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_5114899910098603249.txt};
    \addplot table [x=T,y=Y,select coords between index={46}{46}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_549416532610642337.txt};

  \end{groupplot}
\end{tikzpicture}


==> images/tikz/strategy_power_update_source_files/strategy_power_update_im1.tex <==
%%%%%%%%%%%%%%%%%%%
% Mean-CVaR (PVU) %
%%%%%%%%%%%%%%%%%%%

% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_8873500018088811927.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_3532228027801323971.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_90573412915485638.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_15497166153318989772.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_17698336453125757495.jld2

\begin{tikzpicture}[]
  \begin{groupplot}[
    group style={
        group name=my fancy plots,
        group size=1 by 2,
        xticklabels at=edge bottom,
        vertical sep=0pt
    },
    xtick={1,5,10,15,20,25,30,35,40,47},
    xticklabels={$\tau_{1}$,$\tau_{5}$,$\tau_{10}$,$\tau_{15}$,$\tau_{20}$,$\tau_{25}$,$\tau_{30}$,$\tau_{35}$,$\tau_{40}$,$\tau_{47}$},
    ]

    \nextgroupplot[
    ymin = 0.018, ymax = 0.025,
    xmin = 0, xmax = 48,
    ytick={0.02,0.022,0.024},
    yticklabels={0.02,0.022,0.024},
    xmajorgrids, ymajorgrids,
    scaled ticks=false,
    yticklabel style={
      /pgf/number format/fixed,
      /pgf/number format/precision=5
    },
    y label style={at={(-0.12,0.4)}},
    axis x line=top, 
    axis y discontinuity=parallel,
    height=5.5cm,
    ylabel = Proportion to trade,
    xtick style={draw opacity=0},
    ] 

    \addplot table [x=T,y=Y,select coords between index={0}{45}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_8873500018088811927.txt};
    \addplot table [x=T,y=Y,select coords between index={0}{45}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_3532228027801323971.txt};
    \addplot table [x=T,y=Y,select coords between index={0}{45}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_90573412915485638.txt};
    \addplot table [x=T,y=Y,select coords between index={0}{45}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_15497166153318989772.txt};
    \addplot table [x=T,y=Y,select coords between index={0}{45}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_17698336453125757495.txt};

    \nextgroupplot[
    ymin = -0.002, ymax = 0.012,
    xmin = 0, xmax = 48,
    xmajorgrids, ymajorgrids,
    ytick={0.0,0.005,0.01},
    yticklabels={0.0,0.005,0.01},
    scaled ticks=false,
    yticklabel style={
      /pgf/number format/fixed,
      /pgf/number format/precision=5
    },
    legend pos=south west,
    legend entries={
      $\lambda_{\CVaR} = 0.00$,
      $\lambda_{\CVaR} = 0.25$,
      $\lambda_{\CVaR} = 0.50$,
      $\lambda_{\CVaR} = 0.75$,
      $\lambda_{\CVaR} = 1.00$,
    },
    legend style={at={(0.05,1.0)},anchor=west},
    axis x line=bottom,
    height=3.0cm,
    xlabel = Trading period,
    ]

    \addplot table [x=T,y=Y,select coords between index={46}{46}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_8873500018088811927.txt};
    \addplot table [x=T,y=Y,select coords between index={46}{46}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_3532228027801323971.txt};
    \addplot table [x=T,y=Y,select coords between index={46}{46}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_90573412915485638.txt};
    \addplot table [x=T,y=Y,select coords between index={46}{46}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_15497166153318989772.txt};
    \addplot table [x=T,y=Y,select coords between index={46}{46}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/mean-cvar-optim_17698336453125757495.txt};

  \end{groupplot}
\end{tikzpicture}


==> images/tikz/strategy_power_update_source_files/strategy_power_update_im2.tex <==
%%%%%%%%%%%%%%%%%%
% Mean-CVaR (PU) %
%%%%%%%%%%%%%%%%%%

% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_12345592210445333749.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_7754849124706072148.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_12944883113089842232.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_5114899910098603249.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_549416532610642337.jld2

%%%%%%%%%%%%%%%%%%%
% Mean-CVaR (PVU) %
%%%%%%%%%%%%%%%%%%%

% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_8873500018088811927.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_3532228027801323971.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_90573412915485638.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_15497166153318989772.jld2
% outputs/trading_plan/mean-cvar-optim/mean-cvar-optim_17698336453125757495.jld2

%%%%%%%%%%%%%%
% Difference %
%%%%%%%%%%%%%%

\begin{tikzpicture}[]
  \begin{groupplot}[
    group style={
        group name=my fancy plots,
        group size=1 by 3,
        xticklabels at=edge bottom,
        vertical sep=0pt
    },
    xtick={1,5,10,15,20,25,30,35,40,47},
    xticklabels={$\tau_{1}$,$\tau_{5}$,$\tau_{10}$,$\tau_{15}$,$\tau_{20}$,$\tau_{25}$,$\tau_{30}$,$\tau_{35}$,$\tau_{40}$,$\tau_{47}$},
    xmajorgrids,
    ymajorgrids,
    ytick pos=left,
    ]

    \nextgroupplot[
    separate axis lines,
    axis y discontinuity=parallel,
    axis x line=top, 
    height=3cm,
    ymin = 0.0013,
    ymax = 0.0017,
    xmin = 0, xmax = 48,
    ytick={0.0015,0.0016},
    yticklabels={0.0015,0.0016},
    xtick style={draw opacity=0},
    scaled ticks=false,
    yticklabel style={
      /pgf/number format/fixed,
      /pgf/number format/precision=5
    },
    ]

    \addplot table [x=T,y=Y,select coords between index={46}{46}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_12345592210445333749_mean-cvar-optim_8873500018088811927.txt};
    % \addplot table [x=T,y=Y,select coords between index={46}{46}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_};
    % \addplot table [x=T,y=Y,select coords between index={46}{46}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_};
    % \addplot table [x=T,y=Y,select coords between index={46}{46}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_};
    % \addplot table [x=T,y=Y,select coords between index={46}{46}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_};

    \nextgroupplot[
    % axis x line style={red},
    ymin = -0.0007, ymax = 0.0007,
    xmin = 0, xmax = 48,
    ytick={-0.0005,-0.00025,0.0,0.00025,0.0005},
    yticklabels={-0.0005,-0.00025,0.0,0.00025,0.0005},
    scaled ticks=false,
    yticklabel style={
      /pgf/number format/fixed,
      /pgf/number format/precision=5
    },
    % axis x line=none, 
    separate axis lines,
    x axis line style={draw opacity=0},
    xtick style={draw opacity=0},
    height=5.5cm,
    y label style={at={(-0.15,0.5)}},
    ylabel = Proportion to trade,
    axis y discontinuity=parallel,
    ] 

    \addplot table [x=T,y=Y,select coords between index={0}{45}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_12345592210445333749_mean-cvar-optim_8873500018088811927.txt};
    \addplot table [x=T,y=Y,select coords between index={0}{45}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_7754849124706072148_mean-cvar-optim_3532228027801323971.txt};
    \addplot table [x=T,y=Y,select coords between index={0}{45}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_12944883113089842232_mean-cvar-optim_90573412915485638.txt};
    \addplot table [x=T,y=Y,select coords between index={0}{45}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_5114899910098603249_mean-cvar-optim_15497166153318989772.txt};
    \addplot table [x=T,y=Y,select coords between index={0}{45}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_549416532610642337_mean-cvar-optim_17698336453125757495.txt};

    \nextgroupplot[
    ymin = -0.007, ymax = -0.001,
    xmin = 0, xmax = 48,
    ytick={-0.002,-0.004,-0.006},
    yticklabels={-0.002,-0.004,-0.006},
    scaled ticks=false,
    yticklabel style={
      /pgf/number format/fixed,
      /pgf/number format/precision=5
    },
    legend pos=south west,
    legend entries={
      $\lambda_{\CVaR} = 0.00$,
      $\lambda_{\CVaR} = 0.25$,
      $\lambda_{\CVaR} = 0.50$,
      $\lambda_{\CVaR} = 0.75$,
      $\lambda_{\CVaR} = 1.00$,
    },
    legend style={at={(0.04,3.8)},anchor=west},
    axis x line=bottom,
    height=3.0cm,
    xlabel = Trading period,
    ]

    \addplot table [x=T,y=Y,select coords between index={46}{46}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_12345592210445333749_mean-cvar-optim_8873500018088811927.txt};
    \addplot table [x=T,y=Y,select coords between index={46}{46}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_7754849124706072148_mean-cvar-optim_3532228027801323971.txt};
    \addplot table [x=T,y=Y,select coords between index={46}{46}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_12944883113089842232_mean-cvar-optim_90573412915485638.txt};
    \addplot table [x=T,y=Y,select coords between index={46}{46}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_5114899910098603249_mean-cvar-optim_15497166153318989772.txt};
    \addplot table [x=T,y=Y,select coords between index={46}{46}] {/Users/jvaes/Documents/research/3-implementation/papers/paper1/outputs/txt_files/difference_mean-cvar-optim_549416532610642337_mean-cvar-optim_17698336453125757495.txt};

  \end{groupplot}
\end{tikzpicture}


==> sections/0-abstract_short.tex <==
Optimal trading strategies under price uncertainty have been suggested for liquidating a fixed volume of a single security (Almgren and Chriss).
However this considered volume to trade is often only an estimation,
whose accuracy increases when approaching delivery time.
We thus include volume uncertainty in our model and show that a risk-averse traders' optimal strategy is a trade-off between early and late trades in order to balance risk associated with both price and volume.
By incorporating  a risk term,
our model avoids the explosion in the algorithmic complexity often related to dynamic programming solutions while still yielding competitive performance.

%% Old
%Almgren and Chriss define the optimal trading strategy to liquidate a fixed volume of a single security under price uncertainty.
%However,
%the volume to trade can sometimes only be estimated,
%the accuracy of this estimation increasing when approaching delivery time.
%We thus include volume uncertainty in our model and show that a risk-averse traders’ optimal strategy is a trade-off between early and late trades in order to balance risk associated with both price and volume.
%By incorporating  a risk term,
%our model avoids the explosion in the algorithmic complexity often related to dynamic programming solutions while still yielding competitive performance.


==> sections/7-acknowledgements.tex <==
% \section{Declaration of Interest}%
% \label{sec:declaration_of_interest}

% The authors report no conflicts of interest. The authors alone are responsible for the content and writing of the paper.

\section{Acknowledgements}%
\label{sec:acknowledgements}

% \comadd{We thank the anonymous reviewer for their careful reading and constructive feedback; their input allowed us to improve our paper substantially.}%

The work of the first author was supported by The Alan Turing Institute under the Turing Doctoral Studentship grant TU/C/000022.
The work of the second author was supported by The Alan Turing Institute under the EPSRC grant EP/N510129/1.


==> sources/latex_packages/academicons/README <==
academicons -- high quality icons of online academic profiles

The "academicons" package provides access in (La)TeX to 112 high quality icons
of online academic profiles included in the free "Academicons" font. This
package requires either the Xe(La)TeX or Lua(La)TeX engine to load the
"Academicons" font from the system, which requires installing the bundled
"academicons.ttf" font file. As new releases come out, it is recommended to
install the bundled font version as there may be differences between the package
and previous font versions or newest font versions not yet contemplated in the
package.

The "Academicons" font was designed by James Walsh and released (see
http://jpswalsh.github.io/academicons/) under the open SIL Open Font License
(available at http://scripts.sil.org/OFL). This package is a redistribution of
the free "Academicons" font with specific bindings for (La)TeX. It is inspired
and based on the "fontawesome" package (available at
http://www.ctan.org/pkg/fontawesome).

The academicons package provides the generic "\aiicon" command to access icons,
which takes as mandatory argument the name of the desired icon. It also
provides individual direct commands for each specific icon. The full list of
icons and their respective names and direct commands can be found in the
manual. For example, "\aiicon{googlescholar}" yields the same result as
"\aiGoogleScholar".

academicons (La)TeX package
https://www.ctan.org/pkg/academicons
Version: 1.9.0
Author: Diogo A. B. Fernandes, diogoabfernandes at gmail.com
License: LaTeX Project Public License, version 1.3c

Academicons font
Author: James Walsh
Licence: SIL Open Font License, version 1.1


==> sources/latex_packages/lineno/README <==
README
                      lineno.sty  v4.41
                    fnlineno.sty  v0.55

                         2011-02-16 

The LaTeX package lineno.sty provides line numbers on paragraphs.
After TeX has broken a paragraph into lines there will be line numbers
attached to them, with the possibility to make references through the
LaTeX \ref, \pageref cross reference mechanism.

% Copyright 1995--2003 Stephan I. B"ottcher <boettcher@physik.uni-kiel.de>; 
% Copyright 2002--2005 Uwe L"uck, http://www.contact-ednotes.sty.de.vu, 
%                      for versions 4.x and code from former Ednotes 
% Copyright 2011       Uwe L"uck as above, for fnlineno.sty/tex/pdf
%                      bundle--author-maintained. 
% 
% The files listed below can be redistributed and/or modified under 
% the terms of the LaTeX Project Public License; either 
% version 1.3a of the License, or any later version.
% The latest version of this license is in
%     http://www.latex-project.org/lppl.txt
% We did our best to help you, but there is NO WARRANTY. 

** [ UL: A few festive words on history and responsibility   **
**       are next preceding hard facts as to (see lower)     ** 
**       o `Files'  and                                      ** 
**       o `Installation and usage'.                       ] ** 

2004-09-13 Uwe L"uck  [(UL)]  is new maintainer for lineno.sty. 

lineno.sty served the purpose for which I wrote it years ago.  Uwe
L"uck uses lineno.sty with his Ednotes package, which required quite a
few changes and fixes.  His package depends on lineno, therefore
Uwe agreed to take over the maintenance of lineno.sty.

lineno.sty v4.0 includes most of the well tested changes that Uwe
needs for Ednotes.  These changes blend well into the concepts of the
package, so I am happy to let it go.  

From here on it is Uwe's, and he may proceed to mangle it as he likes.
Expect some radical changes.  You may find him to be quite a bit
friendlier towards the poor souls who still use Windows :-).
Currently, you need some kind of Unix environment to extract the
source documentation from the sty file.

If some version 3 users run into difficulties with Uwe's newer
versions, but need a minor bug-fix in version 3, please do not
hesitate to ask me for help.  But all requests for new features or
major changes shall go to Uwe.

Cheers
Stephan


[ Thanks!  And please let me know as well should 
  compatibility problems arise!  The announced radical 
  changes are postponed again this time (v4.1). 
  --Ednotes is in 
    http://mirror.ctan.org/macros/latex/contrib/ednotes.
                                                   Uwe ] 


Changes: see CHANGEs.txt; earlier:

   2004-10-19  UL: package options for tabular and math 
   2004-09-03  UL: merge Ednotes changes, taking over lineno.sty

   2002 .. 2003 FMi, UL, SiB: bug fixes
   2001-08-04 SiB: linenomath wrapping for \[ \]
   2001-07-30 SiB: [hyperref] option obsolete.
   2001-01-17 SiB: LaTeX class option [twocolumn] support
   2001-01-04 SiB: LaTeX class option [fleqn] support
   2000-12-18 SiB: longtable compatibility
   2000-07-01 SiB: extra \newlabel items, [hyperref] option
   2000-03-10 SiB: indirect call of \output, to work with multicol.
   1999-08-28 SiB: fixed the footnote problem using \holdinginserts
   1999-06-11 SiB: included the extensions into lineno.sty
   1999-03-02 SIB: Added LPPL License


Files (cf. SRCFILEs.txt):

   README.txt    This file.                              (v4.1: UL)
   CHANGEs.txt   Differences to previous versions.       (v4.1: UL)
   COPYING.txt   The LPPL header.
   SCRFILEs.txt  Source file infos                       (UL 2011)
   lineno.sty    The package itself, ready to use.
   edtable.sty   Module for tabular environments.        (UL, v4.1) 
   ednmath0.sty  Module for \linelabel in math mode.     (UL, v4.1) 
   fnlineno.sty  Add-on for footnote line numbers        (UL, v0.55)
   lineno.tex    The source for the documentation (generated)
   lineno.pdf    PDF deriving from the former.           (v4.1: UL)
   lnosuppl.pdf  PDF listing of present non-PDF files 
   ulineno.tex   The pathetic attempt of a users' manual. 
                 [Describes v3.1 currently.]             (UL, v4.1) 
   ulineno.pdf   PDF of former.
   vplref.sty    Conditionally include page number in 
                 line number references                  (UL, v4.2) 

     As of version v3.00, the extension packages for lineno have all been
     incorporated into lineno.sty itself.  Except for itemrule.sty,
     which was removed.

Home:

   http://mirror.ctan.org/macros/latex/contrib/lineno/

TDS version:

   http://mirror.ctan.org/install/macros/latex/contrib/lineno.tds.zip

Authors:

   Uwe L"uck <http://contact-ednotes.sty@web.de>
   Stephan I. B"ottcher <boettcher@physik.uni-kiel.de>

Compatibility with other packages:

   wrapfig.sty   works since v2.05

   multicol.sty  works partly since 3.02.  
                 Do NOT use \linelabel.  Do NOT put a multicol in
                 internal vertical mode {table}, {figure}, etc.

   hyperref.sty  \ref to a \linelabel works since v3.03.

   longtable.sty broke with lineno.sty loaded, but not enabled. 
                 This is fixed in v3.04.

   amsmath.sty   loadable, but not fully supported, with v4.41

Installation and usage (UL, v4.1): 

   For being able to use ALL the new lineno.sty options, the 
   following files must be "visible" to (La)TeX ("visible" 
   explained below for beginners): 

     lineno.sty, edtable.sty, ednmath0.sty, ltabptch.sty 
 
   as above ("Home", note that clicking on "entire directory" 
   suffices); 

     longtable.sty -- from the standard LaTeX Tools bundle. 

   Usage always starts with loading lineno.sty by \usepackage. 
   The remaining .sty files are loaded automatically on the 
   lineno.sty options (and we recommend not to load them through 
   [the mandatory argument of] \usepackage). 
 
   For details, see lineno.tex/pdf and the .sty files mentioned 
   above--search especially for tabular and math mode. 
   (+ `print' below here). 
 
   "Visible to (LaTeX)": Some users don't understand this 
   "visibility" for a while, and indeed it may be somewhat 
   non-trivial. These users may find help in 

      http://mirror.ctan.org/macros/latex/ednotes/visible.txt .

   E.g., former users of lineno.sty may just put all the .sty 
   files into the folder (at their workplace) where they had 
   placed lineno.sty before.                     (/UL, /v4.1)

To print the documented source:

   Take the style-file `lineno.sty', and feed it to a Un*x shell. 
   (Or download the extracted source documentation `lineno.tex'.)

      csh> source ./lineno.sty
      sh>  . ./lineno.sty

   [ I.e., type `sh lineno.sty' (e.g.) as a UNIX command line. 
     Problems with awk may arise. I therefore switched to nawk 
     in lineno.sty v4.00, but this may trouble you as well.    (UL) ] 

   (Please ignore the error message at the beginning about the iffalse.)


Please have a look at a similar work of Michal Jaegermann and James
Fortune:
         http://mirror.ctan.org/obsolete/macros/latex/contrib/numline/





==============================================================================
<- End of official README.txt (UL) 

Changes Feb. 2011: numline obsolete, mirror.ctan.org, fnlineno, 
amsmath compatibility, CHANGEs.txt, lineno.tds.zip
Changes for v4.1 (Oct. 2004): minor fixes (removed `supported/', e.g.); 
bracketed text; lines with `(UL)'; redistribution with README only. 
Formerly: 

                      lineno.sty  v4.0

     $Id: README,v 3.6.2.1 2004/09/13 20:15:47 stephan Exp $

   CTAN:macros/latex/contrib/supported/lineno
         CTAN:macros/latex/contrib/supported/numline/



